Local Equivalences of Graph States

Graph states form a large family of quantum states that are in one-to-one correspondence with mathematical graphs. Graph states are used in many applications, such as measurement-based quantum computation, as multipartite entangled resources. It is thus crucial to understand when two such states have the same entanglement, i.e. when they can be transformed into each other using only local operations. In this case, we say that the graph states are LU-equivalent (local unitary). If the local operations are restricted to the so-called Clifford group, we say that the graph states are LC-equivalent (local Clifford). Interestingly, a simple graph rule called local complementation fully captures LC-equivalence, in the sense that two graph states are LC-equivalent if and only if the underlying graphs are related by a sequence of local complementations. While it was once conjectured that two LU-equivalent graph states are always LC-equivalent, counterexamples do exist and local complementation fails to fully capture the entanglement of graph states. We introduce in this thesis a generalization of local complementation that does fully capture LU-equivalence. Using this characterization, we prove the existence of an infinite strict hierarchy of local equivalences between LC- and LU-equivalence. This also leads to the design of a quasi-polynomial algorithm for deciding whether two graph states are LU-equivalent, and to a proof that two LU-equivalent graph states are LC-equivalent if they are defined on at most 19 qubits. Furthermore, we study graph states that are universal in the sense that any smaller graph state, defined on any small enough set of qubits, can be induced using only local operations. We provide bounds and an optimal, probabilistic construction.

==> fontsets/mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2024/09/14 v1.05 Load Computer/Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Computer Modern text and math fonts (default for pdftex)}
	\RequirePackage[T1]{fontenc} % With T1 encoding, pdftex will silently load the cm-super fontset
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> mydesign.tex <==
\ProvidesFile{mydesign.tex}[2025/01/28 v1.05 Typographic design options for thesis]

%%%%%%%%%%  Color support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color package: xcolor. 
%% Change this if you prefer something else

\usepackage[dvipsnames,svgnames,x11names]{xcolor}

%% can add option [table] to xcolor to use color in tables (see xcolor documentation)


%%%%%%%%%%  Hyperlink and line number colors  %%%%%%%%%%%%%%

\AtBeginDocument{
    % Using color names from xcolor package
    \hypersetup{
		linkcolor=red,
    	citecolor=red,
    	%linkcolor=Blue3,
    	%citecolor=Blue3,
    	urlcolor=violet,
    	filecolor=red, 
    %	anchorcolor=yellow,%  not all pdf viewers recognize this field (although Firefox does): hyperref issues a warning
    %	colorscheme=phelype,% overrides link, cite, url, file colors with a preset scheme, through \DocumentMetadata
    	}
    %
    \ifmit@lineno
	    \renewcommand{\linenumberfont}{\sffamily\mdseries\tiny\color{violet}}% line numbers will be sans-serif, medium weight, tiny, and violet
	\fi
}
